QuantumNAT: Quantum Noise-Aware Training with Noise Injection, Quantization and Normalization

Parameterized Quantum Circuits (PQC) are promising towards quantum advantage on near-term quantum hardware. However, due to the large quantum noises (errors), the performance of PQC models has a severe degradation on real quantum devices. Take Quantum Neural Network (QNN) as an example, the accuracy gap between noise-free simulation and noisy results on IBMQ-Yorktown for MNIST-4 classification is over 60%. Existing noise mitigation methods are general ones without leveraging unique characteristics of PQC; on the other hand, existing PQC work does not consider noise effect. To this end, we present QuantumNAT, a PQC-specific framework to perform noise-aware optimizations in both training and inference stages to improve robustness. We experimentally observe that the effect of quantum noise to PQC measurement outcome is a linear map from noise-free outcome with a scaling and a shift factor. Motivated by that, we propose post-measurement normalization to mitigate the feature distribution differences between noise-free and noisy scenarios. Furthermore, to improve the robustness against noise, we propose noise injection to the training process by inserting quantum error gates to PQC according to realistic noise models of quantum hardware. Finally, post-measurement quantization is introduced to quantize the measurement outcomes to discrete values, achieving the denoising effect. Extensive experiments on 8 classification tasks using 6 quantum devices demonstrate that QuantumNAT improves accuracy by up to 43%, and achieves over 94% 2-class, 80% 4-class, and 34% 10-class classification accuracy measured on real quantum computers. The code for construction and noise-aware training of PQC is available in the TorchQuantum library.

==> texts/postmeasurementpart.tex <==

\subsection{Post-Measurement Normalization}
\label{sec:normalization}
\noindent\textbf{Measurement outcome shift due to quantum noises.}
Before delving into the noise mitigation techniques, we first show analytically how quantum noises influence the \qnn block output. 
The measurement outcomes of the \qnn are sensitive to both the input parameters and any perturbations by some noisy quantum process. 
This section provides insights on such noisy transformations and discusses their impacts on \qnn inference. 

\begin{theorem} \textnormal{(informal version)}\textbf{.} \label{th:linear_noise}
The measurement outcome $y$ of a quantum neural network for the training input data $x$ is transformed by the quantum noise that the system undergoes with a linear map $f(y_x) = \gamma y_x + \beta_x$, where the translation $\beta_x$ depends on the input $x$ and quantum noises, while scaling factor $\gamma$ is input independent.
\end{theorem}

We refer to Appendix Section \ref{proof:linear_noise} for background and a complete proof. The main theoretical contribution of this theorem equips our proposed normalization methodology with robustness guarantees. Most importantly, we observe that the changes in measurement results can often be compensated by proper post-measurement normalization across input batches. For simplicity, we restrict our analysis on $Z$-basis single-qubit measurement outcome $y$. Similar analytical results for multi-qubit general-basis measurement will follow if we apply the same analysis qubit by qubit. Theorem \ref{th:linear_noise} is most powerful when applied on a small batch of input data $\mathbf{x} = \{x_1, \dotsc, x_m\}$ where each $x_i$ is a set of classical input values for the encoder of the QNN and $m$ is the size of the batch. In an ideal noiseless scenario, the QNN model outputs measurement result $y_i$ for each input $x_i$. For a noisy QNN, the measurement result undergoes a composition of two transformations: (1) a constant scaling by $\gamma$; (2) a input-specific shift by $\beta_i$, i.e., $f(y_i) = \gamma y_i + \beta_i$. In the realistic noise regime, the scaling constant $\gamma \in[-1,1]$. However, for small noises, $\gamma$ is close to 1, and $\beta_i$ is close to 0. Therefore, the distribution of noisy measurement results undergoes a constant scaling by $\gamma \leq 1$ and a small shift by each $\beta_i$. In the small-batch regime when $\boldsymbol{\beta} = \{\beta_1, \dotsc, \beta_m\}$ has small variance, the distribution is shifted by its mean $\beta=\E[\boldsymbol{\beta}]$. Thus $f(y_i) \approx \gamma y_i + \beta$. 


\noindent\textbf{Post-measurement normalization}.
Based on the analysis above, we propose \emph{post-measurement normalization} to offset the distribution scaling and shift. 
For each qubit, we collect its measurement results on a batch of input samples, compute their mean and std., then make the distribution of each qubit across the batch \emph{zero-centered} and of \emph{unit variance}. This is performed during both training and inference. 
During training, for a batch of measurement results: $\boldsymbol{y} = \{y_1, \dotsc, y_m\}$, the normalized results are $\hat{ y_{i}}=(y_{i}-\E[\boldsymbol{y}])/\sqrt{\Var(\boldsymbol{y})}$. 
For noisy inference, we correct the error as $\widehat{f(y_{i})}=(f(y_{i})-\E[f(\boldsymbol{y})])/\sqrt{\Var(f(\boldsymbol{y}))} = ((\gamma y_{i} + \beta) - (\gamma \E[\boldsymbol{y}] + \beta)) / \sqrt{\gamma^2\Var(\boldsymbol{y})} = \hat{y_{i}}$.

Figure~\ref{fig:norm} compares the noise-free measurement result distribution of 4 qubits (blue) with their noisy counterparts (yellow) for MNIST-4. Qualitatively, we can clearly observe that the post-measurement normalization reduces the mismatch between two distributions. 
Quantitatively, we adopt signal-to-noise ratio, $SNR = \|\bm{A}\|_{2}^2/\|\bm{A}-\widetilde{\bm{A}}\|_{2}^2$, the inverse of relative matrix distance (RMD), as the metric. The SNR on each qubit and each individual measurement outcome is clearly improved. Though similar, it is different from Batch Normalization~\citep{ioffe2015batch} as the testing batch uses its own statistics instead of that from training, and there is no trainable affine parameter.

